Neural Network-Based Single-Carrier Joint Communication and Sensing: Loss Design, Constellation Shaping and Precoding

We investigate the impact of higher-order modulation formats on the sensing performance of single-carrier joint communication and sensing (JCAS) systems. Several separate components such as a beamformer, a modulator, a target detector, an angle of arrival (AoA) estimator and a communication demapper are implemented as trainable neural networks (NNs). We compare geometrically shaped modulation formats to a classical quadrature amplitude modulation (QAM) scheme. We assess the influence of multi-snapshot sensing and varying signal-to-noise ratio (SNR) on the overall performance of the autoencoder-based system. To improve the training behavior of the system, we decouple the loss functions from the respective SNR values and the number of sensing snapshots, using upper bounds of the sensing and communication performance, namely the Cram\'er-Rao bound for AoA estimation and the mutual information for communication. The NN-based sensing outperforms classical algorithms, such as a Neyman-Pearson based power detector for object detection and ESPRIT for AoA estimation for both the trained constellations and QAM at low SNRs. We show that the gap in sensing performance between classical and shaped modulation formats can be significantly reduced through multi-snapshot sensing. Lastly, we demonstrate system extension to multi-user multiple-input multiple-output to address the improvement of spatial efficiency when servicing multiple user equipments. Our contribution emphasizes the importance of estimation bounds for training neural networks, especially when the trained solutions are deployed in varying SNR conditions.

==> figures/theober_psk.tex <==
esno ber
0   0.335992121473360
1.000000000000000   0.319009235983479
2.000000000000000   0.301237277326305
3.000000000000000   0.282845555866978
4.000000000000000   0.264023021085621
5.000000000000000   0.244966820713618
6.000000000000000   0.225870782130316
7.000000000000000   0.206916250090423
8.000000000000000   0.188267258933389
9.000000000000000   0.170070708029292
10.000000000000000   0.152460478513750
11.000000000000000   0.135562985343067
12.000000000000000   0.119501132945533
13.000000000000000   0.104394287450790
14.000000000000000   0.090353459083530
15.000000000000000   0.077472782305056
16.000000000000000   0.065819830377020
17.000000000000000   0.055427738537166
18.000000000000000   0.046291427650800
19.000000000000000   0.038368809838205
20.000000000000000   0.031586375921330
21.000000000000000   0.025847572295632
22.000000000000000   0.021042092087938
23.000000000000000   0.017054508931661
24.000000000000000   0.013771275665010
25.000000000000000   0.011085714583374
26.000000000000000   0.008901076331795
27.000000000000000   0.007131997475920
28.000000000000000   0.005704774288161
29.000000000000000   0.004556851218732
30.000000000000000   0.003635851420292
31.000000000000000   0.002898391498123
32.000000000000000   0.002308844402081
33.000000000000000   0.001838151720116
34.000000000000000   0.001462740900953
35.000000000000000   0.001163571949549
36.000000000000000   0.000925318587587
37.000000000000000   0.000735677510663
38.000000000000000   0.000584793527844
39.000000000000000   0.000464786029895
40.000000000000000   0.000369361988479
41.000000000000000   0.000293501598139
42.000000000000000   0.000233204135795
43.000000000000000   0.000185283264670
44.000000000000000   0.000147202643031
45.000000000000000   0.000116944204256


==> figures/theober_qam.tex <==
esno ber
0   0.320515727221482
1.000000000000000   0.301290486059434
2.000000000000000   0.281312888009962
3.000000000000000   0.260783430968155
4.000000000000000   0.239909866686782
5.000000000000000   0.218907430974429
6.000000000000000   0.198001922730853
7.000000000000000   0.177432128292356
8.000000000000000   0.157448008297684
9.000000000000000   0.138302445798532
10.000000000000000   0.120236717003781
11.000000000000000   0.103462308303227
12.000000000000000   0.088143289382884
13.000000000000000   0.074383515276292
14.000000000000000   0.062221489889367
15.000000000000000   0.051633465976151
16.000000000000000   0.042543245948795
17.000000000000000   0.034835911075312
18.000000000000000   0.028372539394740
19.000000000000000   0.023003602763531
20.000000000000000   0.018579697492198
21.000000000000000   0.014959167523061
22.000000000000000   0.012012817573791
23.000000000000000   0.009626251356623
24.000000000000000   0.007700470122543
25.000000000000000   0.006151320885258
26.000000000000000   0.004908270716333
27.000000000000000   0.003912856032064
28.000000000000000   0.003117041738235
29.000000000000000   0.002481635134493
30.000000000000000   0.001974834423966
31.000000000000000   0.001570947847204
32.000000000000000   0.001249291879147
33.000000000000000   0.000993260892870
34.000000000000000   0.000789552392016
35.000000000000000   0.000627528514993
36.000000000000000   0.000498694042966
37.000000000000000   0.000396272287578
38.000000000000000   0.000314862159445
39.000000000000000   0.000250161919012
40.000000000000000   0.000198747298671
41.000000000000000   0.000157893707432
42.000000000000000   0.000125434019891
43.000000000000000   0.000099644991490
44.000000000000000   0.000079156641098
45.000000000000000   0.000062880021986

